Real Classification by Description: Extending CLIP's Limits of Part Attributes Recognition

In this study, we define and tackle zero shot "real" classification by description, a novel task that evaluates the ability of Vision-Language Models (VLMs) like CLIP to classify objects based solely on descriptive attributes, excluding object class names. This approach highlights the current limitations of VLMs in understanding intricate object descriptions, pushing these models beyond mere object recognition. To facilitate this exploration, we introduce a new challenge and release description data for six popular fine-grained benchmarks, which omit object names to encourage genuine zero-shot learning within the research community. Additionally, we propose a method to enhance CLIP's attribute detection capabilities through targeted training using ImageNet21k's diverse object categories, paired with rich attribute descriptions generated by large language models. Furthermore, we introduce a modified CLIP architecture that leverages multiple resolutions to improve the detection of fine-grained part attributes. Through these efforts, we broaden the understanding of part-attribute recognition in CLIP, improving its performance in fine-grained classification tasks across six popular benchmarks, as well as in the PACO dataset, a widely used benchmark for object-attribute recognition. Code is available at: https://github.com/ethanbar11/grounding_ge_public.

==> figures/pie.tex <==
\usepackage{pgf-pie}
\begin{tikzpicture}
    \pie{48/plants, 42/Animals, 6.5/Artifact, 1.5/Food, 2/Other }
\end{tikzpicture}

==> sections/deficiency_old_remove.tex <==
% Ethan version
\subsection{Using descriptions for image classification }
% Over the past year and with the emergence of LLMs, it became very common to use LLM generated descriptions with CLIP \cite{menon2022visual, Kaul2023, chen2023ovarnet, more}, in the following manner: \\
% Given a category set $C = \set{c_1,c_2...c_n}$, and for every $c_i$, an LLM is asked to describe $c_i$ visually, and to output $k$ sentences, such that for every class $c_i$ there are $k$ sentences describing it, we'll note them as $d_i$, and remember that $|d_i| = k$. It is important to note here that every description sentence contains the class name in all those methods. \\
% With notating $\phi_V$  as CLIP's image encoder and $\phi_T$ as CLIP's text encoder, the classification for a given image $x$ is determined by: \\
% $c_{pred} = \underset{i}{\mathrm{arg\,max}} \left( \phi_V(x) \cdot \frac{1}{k} \sum_{j=1}^{k} \phi_T(d_{i,j}) \right)$
Over the past year, it has become increasingly common to use Large Language Models (LLMs) for generating descriptions to be inserted into CLIP \cite{menon2022visual, Kaul2023, chen2023ovarnet, more}. \\
Consider a category set \( C = \{c_1, c_2, \ldots, c_n\} \). For each category \( c_i \), an LLM generates \( k \) descriptive sentences, denoted as \( d_i \) with \( |d_i| = k \). Each sentence includes the class name. \\
Using CLIP's image encoder \( \phi_V \) and text encoder \( \phi_T \), the classification of an image \( x \) is given by: \\
\[ c_{pred} = \underset{i}{\mathrm{arg\,max}} \left( \phi_V(x) \cdot \frac{1}{k} \sum_{j=1}^{k} \phi_T(d_{i,j}) \right) \]
The team behind WaffleCLIP~\cite{roth2023waffling} demonstrated that adding random text, instead of LLM-generated text, to the descriptions still improves vanilla CLIP. This led us to question the effect of omitting class names from these descriptions. \\

\subsection{CLIP is bad with descriptions/attributes}
As illustrated in Table \ref{tab:with_vs_without_names_ox} and \ref{tab:with_vs_without_names_col}, and following the method outlined in \ref{alg:filter_name}, we removed the class names from the descriptions in 5 (\textcolor{red}{Insert correct number}) standard fine-grained zero-shot classification datasets. The results, as shown, indicate a significant decrease in performance.

\TODO{I NEED A FIGURE SHOWING HOW CLIP IS FAILING ON SIMPLE THINGS (LENGTH, COLOR, ETC), and then reference it here}


\todo{add figures showing big part vs medium vs small vs whole object, colors,shape, size of description and how good it is}


\subsection{How good can you get with descriptions?}
\textit{A picture is worth a \cancel{16x16} thousand words}
In general, there is an inherent difficulties for describing a picture using text, that is analogous to Kolmogorov complexity - one can describe an image pixel by pixel, but normally for an effective description one uses high level notions that convey complex visual characteristics. Also, CLIP max textual embedding is 77. 

Thus, a question arises - how good can you get by trying to classify an object in a zero-shot manner, using only text description of the object and CLIP? %And to formalize further - Assuming there is the best description set $d^*$ (where $|d^*| = n * k$  (n - classes amount, k- descriptions per class), which for a certain dataset achieves 
After numerous tries, we have come down for two styles of descriptions:
{\bf Oxford Prompting Style} (named after~\cite{Kaul2023}): This style involves generating sentences that describe objects based on their general attributes and parts. The descriptions are more free-form and provide a comprehensive narrative covering various aspects of the object. However, it's noteworthy that the generated sentences tend to be quite repetitive. \TODO{Add example of one image (class) and the two styles.}

{\bf Columbia Prompting Style} (named after~\cite{menon2022visual}): In contrast, the Columbia style adopts a more structured approach. Its descriptions are concise, focusing specifically on a single part and attribute of the object. Unlike the Oxford style, the Columbia style's descriptions are typically non-repetitive, with each description highlighting a different aspect of the object's visual appearance.

\TODO{Insert explanation here why oxford is better, with experiments.}

It is important to highlight that CLIP functions as a late-fusion model. This implies that during the process of computing the latent representation of an image, specifically through \(\phi_V(x)\), the image encoder operates independently of any pertinent textual information that may correspond to the image's content. Prior studies (Add citation here for relevant works) have identified limitations in CLIP's ability to effectively compress images containing multiple objects. However, our focus is on datasets featuring single-object images. Notably, even in these scenarios, CLIP struggles to adequately capture and compress the essential attributes and parts of the object into its latent representation.

% {\bf Oxford Prompting Style} (named after~\cite{Kaul2023}) : This style involves generating sentences that describe objects based on general attributes and parts of attributes. The descriptions are more free-form, providing a comprehensive narrative that encompasses various aspects of the object, and the generated sentences (descriptions) are quite repetitive. \TODO{Add example of one image (class) and the two styles} 

% {\bf Columbia Prompting Style} (named after~\cite{menon2022visual}): In contrast, the Columbia style adopts a more structured approach. Descriptions are concise and focus specifically on a single part and a single attribute of the object, and normally are not repetetive (each description describes different aspect of the visual appearance of the object) %This style challenges the model to accurately classify based on limited yet focused information. It is particularly useful for evaluating the model's efficiency in recognizing key distinguishing features when presented with minimal context. 


% GUY OLD:
%  The conventional approach to classification by description involves associating images with class descriptions, a method that has been highlighted recently by several works (e.g.,\cite{menon2022visual, Kaul2023, chen2023ovarnet, more} \textcolor{red}{I think we should put a lot of citations here, lots of works are doing this} in the study of zero-shot classification by VLMs. Generally, these methods incorporate the object class name within the description, potentially leading to a scenario where the class name itself heavily influences the text-to-image embedding alignment in models like CLIP. This raises a concern that the rest of the description may become secondary, and the classification accuracy might be predominantly driven by the class name, now embedded within a broader textual context. This hypothesis, which we propose and explore, finds support in recent studies such as WaffleCLIP~\cite{roth2023waffling} and the analysis of CLIP as a 'Bag-of-Words'\cite{yuksekgonul2022and}, both of which examine the actual contribution of attribute-based descriptions beyond the class name in the process of classification by description.

% To substantiate our claim, we conducted a series of experiments in which we intentionally omit the object class name from the descriptions used in recent works. Our findings, shown in Table~\ref{XX}, reveal a dramatic decrease in the efficacy of zero-shot classification by description, underscoring the significant role object names play in current VLM methodologies and challenging the assumption that these models deeply understand the full spectrum of descriptive attributes. Figure~\ref{XX} illustrates this phenomenon. 
 
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/figure_classification_by_description.png}}
\caption{Examples showing the decrease in classification performance when removing object name from description. \TODO{replace figure}}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}


\input{tables/table_with_and_without_names_ox}
\input{tables/table_with_and_without_names_col}


 % UP TO HERE



% \cite{roth2023waffling}

% {\bf Ethan}
% Each here should be a paragraph


\begin{itemize}
    % \item Explain how you normally do image classification with class descriptions (and reference Vondrick's and other works in the field)

    % \item Show that by removing the name from each of the papers, (analogous to what WaffleCLIP did), the results decrease dramatically (insert table/figure to reference to)

    % \item Example showing specific descriptions and how he fails on them, maybe a short debate regarding the best and worst descriptions - maybe CLIP is better on big items and worse on small? maybe he is better on short sentences/large? Insert here reference to CLIP as bag of words
    % \begin{itemize}
    %     \item Figure showing specific example and how CLIP fails on it
    %     \item figure Big parts vs medium vs small vs whole object
    %     \item figure - colors, shape, size
    % \end{itemize}
    % \item Prompting
    % \begin{itemize}
    % \item Some formality about prompting, and debate regarding the ceiling of prompting & kolmogorov complexity
    %     \item We tested two "families" of prompts, both present in earlier papers
    %     \item Tested many prompt styles
    %     \item Shown are the best we received
    %     \item \TODO{Prompt tuning if we have time?}
    % \end{itemize}
    % \item Also reference here the post-fusion deficiency.

    % \item Explain what we've done to get the "best" prompts with CLIP, to prove it is really bad with descriptions and it's not just our bad prompts. \textcolor{red}{Maybe prompt tuning example here on a specific small dataset? They should be convinced in this stage that this method is bad without the name}
    % \item Some formality should be here, referencing two inherent deficiencies of CLIP - post-fusion (meaning everything should be merged into 1 vector and thus it makes sense to lose information, also reference the retrieval training regime) & text based classification (the inability of textual description to classify all there is). \textcolor{red}{At the end, we need to show how well is our fine tuned version on normal ImageNet1k/standard datasets.}
    

\end{itemize}

==> sections/exp_old.tex <==
% experiments
\label{sec: exp}
In this section, we detail the experiments conducted to evaluate the efficacy of our fine-tuned CLIP model. Our tests were carried out on a selection of datasets that are standard in the field of fine-grained classification. These datasets were chosen for their relevance and consistency in benchmarking performance in this domain. Specifically, they require visual understanding of parts and attributes. 
\TODO{Add citations for datasets}
{\bf CUB (Caltech-UCSD Birds-200-2011)}: This dataset is a collection of 200 bird species with high inter-class similarity, making it a challenging dataset for fine-grained classification that is based on description. 

{\bf Flowers102}: Comprising 102 categories of flowers common to the UK, this dataset is characterized by its large intra-class variation and minimal inter-class differences. It tests the model's ability to discern subtle differences in floral structures.

{\bf Cars196}: Featuring 196 car models, this data set provides a diverse range of automobiles with variations in design, model year, and manufacturer. It challenges the model to recognize and differentiate between fine details in vehicle designs.

{\bf Food101}: This dataset contains 101 food categories, each class having 1,000 images. The diversity of food items, ranging from fruits to complex dishes, tests the model’s ability to classify images based on varied textures, ingredients and presentation styles.

{\bf Dogs120}: Consisting of 120 breeds of dogs, this dataset is particularly useful for evaluating the model's performance in classifying animals with high visual similarity. It requires the model to pay attention to subtle differences in fur patterns, colors, and body shapes.

{\bf OxfordPets}: The Oxford-IIIT Pet dataset includes 37 categories of pets, with roughly equal representation of cats and dogs. It challenges the model to distinguish between a wide range of pet breeds, focusing on fine-grained features and differences in animal appearances.

Each of these datasets provides a unique set of challenges in fine-grained classification, ranging from subtle differences in species, breeds, or models, to variations in colors, shapes, and textures. 

\sebsection{Finetuned vs/. Baseline Results with Standard CLIP Models}
% Before presenting the results of our fine-tuned model, it is essential to establish a baseline for comparison. To this end, we first document the performance of standard CLIP models on our selected benchmarks. This includes results obtained using various prompting styles and different model backbones, providing a comprehensive view of the model's capabilities in its original state.

% To compare baseline CLIP models with fine-tuned ones, we employed two distinct prompting styles to understand their impact on model performance in fine-grained classification tasks. These styles were chosen to represent different approaches to describing objects and their attributes. Following the discussion in Sec.~\ref{lebl:deficiency}, the so-called Oxford and Columbia prompting styles were selected. 

% {\bf Oxford Prompting Style} (named after~\cite{Kaul2023}) : This style involves generating sentences that describe objects based on general attributes and parts of attributes. The descriptions are more free-form, providing a comprehensive narrative that encompasses various aspects of the object. This style tests the model's ability to understand and synthesize broader and more holistic descriptions, which are crucial for distinguishing between closely related categories in fine-grained classification tasks.

% {\bf Columbia Prompting Style} (named after~\cite{menon2022visual}): In contrast, the Columbia style adopts a more structured approach. Descriptions are concise and focus specifically on a single part and a single attribute of the object. This style challenges the model to accurately classify based on limited yet focused information. It is particularly useful for evaluating the model's efficiency in recognizing key distinguishing features when presented with minimal context. 

Alongside these prompting styles, we also tested different backbones of the CLIP model. The detailed results of these experiments, which compare the baseline performance of standard CLIP models with our fine-tuned version across various datasets and CLIP backbones, are presented in Table~\ref{tab:classification_results_ox} for the Oxford prompting style and in Table~\ref{tab:classification_results_col} for the Columbia prompting style. These tables reveal a significant gap in accuracy between baseline and fine-tuned versions. 

\subsection{Fine-Tuning Process of CLIP Model}
{\bf Data selection.} Our fine-tuning process began with careful selection of data. As mentioned above, we chose $K=20$ images from each category of the class in ImageNet21k, accompanied by $N=10$ unique sentences describing their attributes, resulting in $NxK$ image-text pairs for each class. This selection was made to ensure a rich diversity in the training data, exposing the model to a wide range of object attributes and descriptions. 
To capture the vast diversity within our dataset, we organized the class names into broader super categories such as Animals and Insects, Plants and Fungi, Man-Made Objects, and Natural Objects and Geographical Features. This classification facilitates a comprehensive and non-overlapping representation of the myriad of entities, ranging from various species of flora and fauna to a wide array of human-made and natural objects, enhancing the model's ability to recognize and describe a broad spectrum of subjects accurately.

\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/classes_pie_plot.png}}
\caption{A plot showing the distribution of classes taken from ImageNet21k for training. The reason why plants and animals are dominant is because there are multiple sub-categories for these two types in ImageNet21k. These sub-categories are beneficial for our training purposes, since LLMs can provide a rich set of essential features for them.}
\label{fig:imagenet21k_distribution_training}
\end{center}
\vskip -0.2in
\end{figure}


{\bf Hyperparameter Settings.} 
In the fine-tuning of CLIP for enhanced attribute learning, we carefully selected specific hyperparameters based on preliminary experiments and literature benchmarks to optimize training efficiency and model performance. The initial learning rate was set at $10^{-5}$ and was accompanied by a decay schedule for gradual reduction. We have used a scheduling policy of CosineAnnealingLR, with 10000 warmup steps. We chose a batch size of 400, for sufficiently diverse classes, as well as computational efficiency and effective learning. For the optimization process, we employed the AdamW optimizer and incorporated a weight decay of 0.1 to enhance the model's generalization capabilities. The OpenCLIP framework was utilized, and we performed fine-tuning based on the 'openai' checkpoint as it yielded the best outcomes in the preliminary experiments.

{\bf Evaluation. } Post-training, the fine-tuned model's performance was evaluated using the accuracy metrics of the top1 and top5. These metrics provided a comprehensive assessment of the model's classification capabilities on the fine-grained classification tasks.

\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/figure_classification_by_description.png}}
\caption{Placeholder for figure. \TODO{plots generated by test ovoc after training, showing improvement in detection of part attributes.}}
\label{fig:imagenet21k_distribution_training}
\end{center}
\vskip -0.2in
\end{figure}


\subsection{Analysis}
\TODO{[Ethan/Idan/Guy] 
Here, we analyze the results, focusing on how and why the use of semantic descriptions impacts the model’s performance:
Options are: diversity and size of different classes, size of descriptions pet class, description style, etc. 
WE can debate over the prompt effectiveness - how the prompts can be quite noisy, and how it affects the fine tuning (we have noise but it still works)
Ablations of:
- diversity of classes/size
- with/without smart batching other methods
- Negative minings?
    - Training on one prompt and testing on the other
- Showing that CLIP is worse/better with attributes of big parts? what attributes is he good with?
}

% {\bf Ethan}
% \begin{itemize}
%     \item Go over the datasets we test on, explaining they are standard in fine-grained classification, comparing in table original vs finetuned.
%     \item Go over the finetune process
%     \item Debate over the prompt effectiveness - how the prompts can be quite noisy, and how it affects the fine tuning (we have noise but it still works)
%     \item Different subsets of ImageNet21k classes - how we choose them.
%     \item Ablations of:
% 	- diversity of classes/size
% 	- with/without smart batching other methods
% 	- Negative minings?
%         - Training on one prompt and testing on the other
% 	- Showing that CLIP is worse/better with attributes of big parts? what attributes is he good with?
% \end{itemize} 

% {\bf Guy}
% \subsection{Comparing baselines on real-zero shot}
% Here we show the baseline results from standard CLIP models on our benchmarks. We show include various prompting styles and various backbones

% \subsection{Results for enhancing CLIP training with semantic object descriptions}
% we show here the results of our experiments and highlight the improvements in the accuracy of the zero-shot classification.

% \subsection{Analysis}
% Here, we analyze the results, focusing on how and why the use of semantic descriptions impacts the model’s performance:
% Options are: diversity and size of different classes, size of descriptions pet class, description style, etc. 


\input{tables/table_baseline_vs_finetuned_ox}
\input{tables/table_baseline_vs_finetuned_col}




==> sections/neurips_checcklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper has no theoretical result
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We release code and detail the full experimental setup and steps to recreate experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We append an annonymized version of the code
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:We detail the experimental setup and release the code in anonymized way.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided the relevant information in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't foresee any negative societal impact, while the positive one is obviously contributing to the scientific community. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No risks
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \anwerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite the original paper when using them.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

